Formal Evidence Generation for Assurance Cases for Robotic Software Models

Robotics and Autonomous Systems are increasingly deployed in safety-critical domains, so that demonstrating their safety is essential. Assurance Cases (ACs) provide structured arguments supported by evidence, but generating and maintaining this evidence is labour-intensive, error-prone, and difficult to keep consistent as systems evolve. We present a model-based approach to systematically generating AC evidence by embedding formal verification into the assurance workflow. The approach addresses three challenges: systematically deriving formal assertions from natural language requirements using templates, orchestrating multiple formal verification tools to handle diverse property types, and integrating formal evidence production into the workflow. Leveraging RoboChart, a domain-specific modelling language with formal semantics, we combine model checking and theorem proving in our approach. Structured requirements are automatically transformed into formal assertions using predefined templates, and verification results are automatically integrated as evidence. Case studies demonstrate the effectiveness of our approach.

==> Implementation_and_tool_support.tex <==
\vspace{-8pt}
\section{Implementation and tool support}
\label{impl}



\begin{table*}[ht]
\caption{Status of tool support for the steps in AC process}
\label{table2}\centering
\begin{small}
\begin{tabular}{|c|l|l|l|}
\hline
No. & Step                                                       & Automated/ manual & Tool support                        \\
\hline
1   & AC Claim structuring               & Manual           & Kapture                             \\
\hline
2   & DSL Assertion generation from XML claims & Automated        & Epsilon/ EGL                         \\
\hline
3   & Model checking                               & Automated        & RoboTool/ FDR\&PRISM                 \\
\hline
4   & Evidence model generation and integration   & Automated        & Epsilon/ EOL                         \\
\hline

\end{tabular}
\end{small}
\end{table*}

According to Fig.~\ref{fig: model checking evidence method}, the method outlined in Sect.~\ref{sec:model_checking} consists of four distinct steps. Step 1 involves manual processes, whereas Step 3 is fully implemented by RoboTool and does not contribute to our work. A comprehensive summary of the tasks associated with each step and the corresponding supporting tools is provided in Table~\ref{table2}.
The implementation is developed within the Eclipse EMF framework and relies on three tools: RoboTool\noindent{\footnote{\url{https://www.cs.york.ac.uk/robostar/robotool/}}}, Epsilon\noindent{\footnote{\url{http://download.eclipse.org/epsilon/updates/2.2/}}}, and Kapture\noindent{\footnote{\url{https://www.drisq.com/product-kapture}}}.


RoboTool, an Eclipse plugin, functions as a modelling environment for RoboChart and integrates FDR and PRISM model checkers to enable formal verification. It provides support for generating formal semantics from RoboChart models, converting assertions in RoboChart assertion languages into formal assertions, and retrieving model checking results by invoking the model checkers. 
Epsilon is used to facilitate the transformation process, converting XML claims into RoboChart DSL assertions and translating model checking results into SACM evidence models. Additionally, Kapture is employed to organize and export claims into XML files.

The implementation of the approach in Sect.~\ref{sec:model_checking} and the two case studies discussed in the next section are available online\footnote{\url{https://github.com/laila-fangyan/AC_using_FV.git}}.

==> acronym.tex <==
\newacronym{ras}{RAS}{Robotics and Autonomous System}

\newacronym{oas}{OAS} {Open Adaptive System}

\newacronym{ai}{AI}{artificial intelligence}

\newacronym{ac}{AC}{Assurance Case}

\newacronym{mbe}{MBE}{Model-Based Engineering}

\newacronym{gsn}{GSN}{Goal Structuring Notation}


\newacronym{cae}{CAE}{Claims-Arguments-Evidence}

\newacronym{sacm}{SACM}{Structured Assurance Case Meta-Model}

\newacronym{d-mils}{D-MILS}{Distributed Multiple Independent Levels of Security/Safety}

\newacronym{tim}{TIM}{Traceability Information Model}

\newacronym{osate}{OSATE}{Open Source AADL Tool Environment} 

\newacronym{oslc}{OSLC}{Open Services for Lifecycle Collaboration}

\newacronym{rdf}{RDF}{Resource Description Framework} 

\newacronym{tclt}{TCLT}{Timed Computation Tree Logic}

\newacronym{sysml}{SysML}{Systems Modeling Language} 

\newacronym{tasm}{TASM}{Timed Abstract State Machines} 

\newacronym{bip}{BIP}{Behaviour Interaction Priority}


 \newacronym{hai}{HAI}{Human-automation Interaction}
 
 
 
\newacronym{ltl}{LTL}{Linear Temporal Logic} 


\newacronym{sal-smc}{SAL-SMC}{Symbolic Analysis Laboratory's Symbolic Model Checker}

\newacronym{eofm}{EOFM}{Enhanced Operator Function Model} 
